Approximated Likelihood Ratio: A Forward-Only and Parallel Framework for Boosting Neural Network Training

Efficient and biologically plausible alternatives to backpropagation in neural network training remain a challenge due to issues such as high computational complexity and additional assumptions about neural networks, which limit scalability to deeper networks. The likelihood ratio method offers a promising gradient estimation strategy but is constrained by significant memory consumption, especially when deploying multiple copies of data to reduce estimation variance. In this paper, we introduce an approximation technique for the likelihood ratio (LR) method to alleviate computational and memory demands in gradient estimation. By exploiting the natural parallelism during the backward pass using LR, we further provide a high-performance training strategy, which pipelines both the forward and backward pass, to make it more suitable for the computation on specialized hardware. Extensive experiments demonstrate the effectiveness of the approximation technique in neural network training. This work underscores the potential of the likelihood ratio method in achieving high-performance neural network training, suggesting avenues for further exploration.

==> Figs/acc_acc.tex <==
\begin{figure}[t]
\vspace{-4mm}
    \begin{minipage}[b]{\linewidth} %0.23为minipage的宽度，可以调节子图间的距离
    \includegraphics[width=\linewidth]{Figs/hybrid_lr_cos_list.pdf}\vspace{1pt} %图片的宽度、路径和垂直间距
    \includegraphics[width=\linewidth]{Figs/hybrid_cos_list.pdf}\vspace{1pt}
    %\vspace要紧跟在对应的includegraphics，不然得不到想要的结果
    \end{minipage}
\caption{Gradient estimation accuracy of the Hybrid and approximated Hybrid for ResNet-5. The first figure presents the cosine similarity between the gradients computed by backpropagation and the approximated method, while the second one presents the comparison between the Hybrid and approximated Hybrid methods. }
\label{fig:gradient_acc}
\end{figure}
